Unmasking Transformers: A Theoretical Approach to Data Recovery via Attention Weights

In the realm of deep learning, transformers have emerged as a dominant architecture, particularly in natural language processing tasks. However, with their widespread adoption, concerns regarding the security and privacy of the data processed by these models have arisen. In this paper, we address a pivotal question: Can the data fed into transformers be recovered using their attention weights and outputs? We introduce a theoretical framework to tackle this problem. Specifically, we present an algorithm that aims to recover the input data $X \in \mathbb{R}^{d \times n}$ from given attention weights $W = QK^\top \in \mathbb{R}^{d \times d}$ and output $B \in \mathbb{R}^{n \times n}$ by minimizing the loss function $L(X)$. This loss function captures the discrepancy between the expected output and the actual output of the transformer. Our findings have significant implications for the Localized Layer-wise Mechanism (LLM), suggesting potential vulnerabilities in the model's design from a security and privacy perspective. This work underscores the importance of understanding and safeguarding the internal workings of transformers to ensure the confidentiality of processed data.

==> Hessian_case1.tex <==
\section{Hessian of Case 1}

\subsection{Hessian of \texorpdfstring{\alpha(X)_{i_0}}{}}

\begin{lemma}
If the following conditions
\begin{itemize}
    \item $i_0 = i_1 = i_2 \in [n]$.
    \item Let $W = K^\top Q \in \R^{d \times d}$ (for convenient)
    \begin{itemize}
        \item For each $j_1, j_2 \in [d]$, we use $W_{j_1,j_2}$ to denote the $(j_1,j_2)$-th entry of $W \in \R^{d \times d}$
    \end{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
\end{itemize}
Then we have  
\begin{itemize}
\item Part 1.
\begin{align*}
    \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} }
    = & ~ u(X)_{i_1,i_1} ( Z_{j_1,i_1}^2 + 2 Y_{j_1,i_1} Z_{j_1,i_1} + 2 W_{j_1,j_1} ) \\
    & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle
\end{align*}
\item Part 2. $j_1 \neq j_2$  
\begin{align*}
     \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_2} }
    = & ~  u(X)_{i_1,i_1} (Z_{j_1, i_1} Z_{j_2,i_1} + Y_{j_1,i_1} Z_{j_2,i_1}+Y_{j_2,i_1} Z_{j_1,i_1} + W_{j_1,j_2}+W_{j_2,j_1} )\\
    & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_2},{\bf 1}_n \rangle 
\end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
 
    {\bf Proof of Part 1.}
    \begin{align*}
    & ~ \frac{ \d \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} } \\
        = & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_1} } \\
        = & ~  \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)_{i_1} } { \d x_{i_1, j_1}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} ( u(X)_{i_1,i_1} Z_{j_1,i_1} + \langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} ( u(X)_{i_1,i_1} Z_{j_1,i_1}) + \frac{ \d}{ \d x_{i_1, j_1}}(\langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1}(Z_{j_1, i_1}^2 +  Y_{j_1,i_1}Z_{j_1,i_1} + W_{j_1,j_1} ) + \frac{ \d}{ \d x_{i_1, j_1}}(\langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1}(Z_{j_1, i_1}^2 +  Y_{j_1,i_1}Z_{j_1,i_1} + W_{j_1,j_1} ) \\
        & ~ +  u(X)_{i_1,i_1} ( Z_{j_1,i_1} Y_{j_1,i_1} + W_{j_1,j_1} )  + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle \\
        = & ~ u(X)_{i_1,i_1} ( Z_{j_1,i_1}^2 + 2 Y_{j_1,i_1} Z_{j_1,i_1} + 2 W_{j_1,j_1} ) + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle
    \end{align*}

where the 1st step from $i_0 = i_1 = i_2$, the 2nd step follows from simple algebra, the 3rd step follows from Lemma~\ref{lem:alpha}, the 4th step follows from Fact~\ref{fac:basic_calculus}, the 5th step follows from Lemma~\ref{lem:gradientUZ}, the 6th step follows from Lemma~\ref{lem:gradientUY_1n}.

    {\bf Proof of Part 2.}

We can show that
\begin{align*}
        & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } \\
        = & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)_{i_1} } { \d x_{i_1, j_2}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1,j_1 }} (u(X)_{i_1,i_1}  Z_{j_2,i_1}) + \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } } (\langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1} Z_{j_2,i_1} + \langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle \\
        & ~ + \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } } (\langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle) \\
        =& ~ u(X)_{i_1,i_1}\cdot (Z^2_{j_2, i_1} +  Y_{j_2,i_1} Z_{j_2,i_1}+ W_{j_2,j_2})\\
        & ~ + u(X)_{i_1,i_1} \cdot ( Z_{j_2,i_1} Y_{j_2,i_1} +  W_{j_2,j_2} ) + \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2},{\bf 1}_n \rangle \\
        = & ~ u(X)_{i_1,i_1} (Z^2_{j_2, i_1} + 2Y_{j_2,i_1} Z_{j_2,i_1} + 2W_{j_2,j_2} )+ \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2},{\bf 1}_n \rangle 
\end{align*}

where the 1st step from $i_0 = i_1 = i_2$, the 2nd step follows from simple algebra, the 3rd step follows from Lemma~\ref{lem:alpha}, the 4th step follows from Fact~\ref{fac:basic_calculus}, the 5th step follows from Lemma~\ref{lem:gradientUZ}, the 6th step follows from Lemma~\ref{lem:gradientUY_1n}.
\end{proof}



\newpage
\subsection{Helpful Lemma for Case 1}

\begin{lemma}[$j_1=j_2$ case]
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
\end{itemize}
We have
\begin{itemize}
    \item {\bf Part 1.} 
    \begin{align*}
        Z_{j_1,i_1}^2 = e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_1}
    \end{align*}
    \item {\bf Part 2.}
    \begin{align*}
            2 Y_{j_1,i_1} Z_{j_1,i_1} = e_{j_1}^\top ( W^\top x_{i_1} x_{i_1}^\top W^\top + W x_{i_1} x_{i_1}^\top W ) e_{j_1}
    \end{align*} 
    \item {\bf Part 3.}
    \begin{align*}
        2 W_{j_1,j_1} = e_{j_1}^\top ( W + W^\top ) e_{j_1}
    \end{align*}
    \item {\bf Part 4.}
    \begin{align*}
        \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1} , {\bf 1}_n \rangle = e_{j_1}^\top ( W^\top X \diag( u(X)_{i_1} ) X^\top W )  e_{j_1}
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}

{\bf Proof Part 1.}

We can show
\begin{align*}
 Z_{j_1,i_1}^2 = & ~ e_{j_1}^\top W x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
    = & ~ e_{j_1}^\top W x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_1}  \\
    = & ~ e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 2.}
On one hand
\begin{align*}
  Y_{j_1, i_1} Z_{j_1, i_1} = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_1} 
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}).

On the other hand
\begin{align*}
  Y_{j_1, i_1} Z_{j_1, i_1} 
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W x_{i_1} \cdot  e_{j_1}^\top W^\top x_{i_1}\\
  = & ~ e_{j_1}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from commutative (Fact~\ref{fac:basic_calculus}), the 3rd step follows from $u^\top v = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}).

{\bf Proof of Part 3.}
It is trivial.

{\bf Proof of Part 4.}
We can show
\begin{align*}
    & ~ \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1} , {\bf 1}_n \rangle\\
    = & ~ \langle u(X)_{i_1} \circ Y_{j_1} , Y_{j_1} \rangle \\
    = & ~ Y_{j_1}^\top (u(X)_{i_1} \circ Y_{j_1}) \\
    = & ~ Y_{j_1}^\top \diag( u(X)_{i_1} )Y_{j_1} \\
    = & ~ e_{j_1}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_1}
\end{align*}

where the 1st step follows from $\langle u \circ v,w\rangle = \langle u \circ v \circ w,{\bf 1}_n \rangle$ (Fact~\ref{fac:basci_algebra}), the 2nd step follows from $v^\top u = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from $u^\top(v \circ w) = u^\top \diag(v)w$ (Fact~\ref{fac:basci_algebra}), the 4th step follows from Definition~\ref{def:Y}.
 

\end{proof}

\begin{lemma}[$j_1\neq j_2$]
 
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
\end{itemize}
We have \Zhao{Your $j_1$ and $j_2$ need to showup both in both sides of the below equation}
\begin{itemize} 
    \item {\bf Part 1.} 
    \begin{align*}
        Z_{j_1,i_1} Z_{j_2,i_1} = e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top ) e_{j_2}
    \end{align*}
    \item {\bf Part 2.}
    \begin{align*}
        Y_{j_1,i_1} Z_{j_2,i_1} = e_{j_1}^\top (W^\top x_{i_1} x_{i_1}^\top W^\top)e_{j_2} 
    \end{align*} 
    \item {\bf Part 3.}
    \begin{align*}
    Y_{j_2, i_1} Z_{j_1, i_1} = e_{j_2}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
    \end{align*}
    \item {\bf Part 4.}
    \begin{align*}
        2 W_{j_2,j_2} = e_{j_2}^\top ( W + W^\top ) e_{j_2}
    \end{align*}
    \item {\bf Part 5.}
    \begin{align*}
        \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2} , {\bf 1}_n \rangle = e_{j_2}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_2} 
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
 

{\bf Proof Part 1.}

We can show
\begin{align*}
Z_{j_1,i_1} Z_{j_2,i_1} = & ~ e_{j_1}^\top W x_{i_1} \cdot e_{j_2}^\top W x_{i_1} \\
 = & ~ e_{j_1}^\top W x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_2} \\
 = & ~ e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_2}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 2.}
\begin{align*}
   Y_{j_1,i_1} Z_{j_2,i_1} = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_2}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_2} \\
  = & ~ e_{j_1}^\top (W^\top x_{i_1} x_{i_1}^\top W^\top)e_{j_2} 
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 3.}
\begin{align*}
  Y_{j_2, i_1} Z_{j_1, i_1} 
  = & ~ e_{j_2}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_2}^\top W x_{i_1} \cdot  e_{j_1}^\top W^\top x_{i_1}\\
  = & ~ e_{j_2}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra})

{\bf Proof of Part 4.}
It is trivial.

{\bf Proof of Part 5.}
We can show
\begin{align*}
    & ~ \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2} , {\bf 1}_n \rangle\\
    = & ~ \langle u(X)_{i_1} \circ Y_{j_2} , Y_{j_2} \rangle \\
    = & ~ Y_{j_2}^\top (u(X)_{i_1} \circ Y_{j_2}) \\
    = & ~ Y_{j_2}^\top \diag( u(X)_{i_1} )Y_{j_2} \\
    = & ~ e_{j_2}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_2}
\end{align*}

where the 1st step follows from $\langle u \circ v,w\rangle = \langle u \circ v \circ w,{\bf 1}_n \rangle$ (Fact~\ref{fac:basci_algebra}), the 2nd step follows from $v^\top u = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from $u^\top(v \circ w) = u^\top \diag(v)w$ (Fact~\ref{fac:basci_algebra}), the 4th step follows from Definition~\ref{def:Y}.
\end{proof}

\begin{lemma}[Matrix version for Hessian]
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
    \item Let 
    \begin{align*}
        H = u(X)_{i_1,i_1} \cdot W x_{i_1} x_{i_1}^\top W^\top + W^\top x_{i_1} x_{i_1}^\top W
    \end{align*}
\end{itemize}
We have
\begin{itemize}
 \item {\bf Part 1.} 
    \begin{align*}
        \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } 
        =  e_{j_1}^\top H e_{j_2}
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
It is obvious by combining Lemma ???,....
\end{proof}

==> app_more_related.tex <==
\section{More Related Works}

==> hessian_alpha.tex <==
\section{Hessian}

\iffalse
\subsection{Hessian of Case 1 subblock}

\begin{lemma}
If the following conditions
\begin{itemize}
    \item $i_0 = i_1 = i_2 \in [n]$.
    \item Let $W = K^\top Q \in \R^{d \times d}$ (for convenient)
    \begin{itemize}
        \item For each $j_1, j_2 \in [d]$, we use $W_{j_1,j_2}$ to denote the $(j_1,j_2)$-th entry of $W \in \R^{d \times d}$
    \end{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
\end{itemize}
Then we have  
\begin{itemize}
\item Part 1.
\begin{align*}
    \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} }
    = & ~ u(X)_{i_1,i_1} ( Z_{j_1,i_1}^2 + 2 Y_{j_1,i_1} Z_{j_1,i_1} + 2 W_{j_1,j_1} ) \\
    & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle
\end{align*}
\item Part 2. $j_1 \neq j_2$  
\begin{align*}
     \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_2} }
    = & ~  u(X)_{i_1,i_1} (Z_{j_1, i_1} Z_{j_2,i_1} + Y_{j_1,i_1} Z_{j_2,i_1}+Y_{j_2,i_1} Z_{j_1,i_1} + W_{j_1,j_2}+W_{j_2,j_1} )\\
    & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_2},{\bf 1}_n \rangle 
\end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
 
    {\bf Proof of Part 1.}
    \begin{align*}
    & ~ \frac{ \d \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} } \\
        = & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_1} } \\
        = & ~  \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)_{i_1} } { \d x_{i_1, j_1}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} ( u(X)_{i_1,i_1} Z_{j_1,i_1} + \langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} ( u(X)_{i_1,i_1} Z_{j_1,i_1}) + \frac{ \d}{ \d x_{i_1, j_1}}(\langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1}(Z_{j_1, i_1}^2 +  Y_{j_1,i_1}Z_{j_1,i_1} + W_{j_1,j_1} ) + \frac{ \d}{ \d x_{i_1, j_1}}(\langle u(X)_{i_1} \circ Y_{j_1} , {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1}(Z_{j_1, i_1}^2 +  Y_{j_1,i_1}Z_{j_1,i_1} + W_{j_1,j_1} ) \\
        & ~ +  u(X)_{i_1,i_1} ( Z_{j_1,i_1} Y_{j_1,i_1} + W_{j_1,j_1} )  + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle \\
        = & ~ u(X)_{i_1,i_1} ( Z_{j_1,i_1}^2 + 2 Y_{j_1,i_1} Z_{j_1,i_1} + 2 W_{j_1,j_1} ) + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle
    \end{align*}

where the 1st step from $i_0 = i_1 = i_2$, the 2nd step follows from simple algebra, the 3rd step follows from Lemma~\ref{lem:alpha}, the 4th step follows from Fact~\ref{fac:basic_calculus}, the 5th step follows from Lemma~\ref{lem:gradientUZ}, the 6th step follows from Lemma~\ref{lem:gradientUY_1n}\Yichuan{What about the 7th step?}.

    {\bf Proof of Part 2.}

We can show that
\begin{align*}
        & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } \\
        = & ~ \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)_{i_1} } { \d x_{i_1, j_2}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1,j_1 }} (u(X)_{i_1,i_1}  Z_{j_2,i_1}) + \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } } (\langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle) \\
        = & ~ u(X)_{i_1,i_1} Z_{j_2,i_1} + \langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle \\
        & ~ + \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } } (\langle u(X)_{i_1,} \circ Y_{j_2}, {\bf 1}_n \rangle) \\
        =& ~ u(X)_{i_1,i_1}\cdot (Z^2_{j_2, i_1} +  Y_{j_2,i_1} Z_{j_2,i_1}+ W_{j_2,j_2})\\
        & ~ + u(X)_{i_1,i_1} \cdot ( Z_{j_2,i_1} Y_{j_2,i_1} +  W_{j_2,j_2} ) + \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2},{\bf 1}_n \rangle \\
        = & ~ u(X)_{i_1,i_1} (Z^2_{j_2, i_1} + 2Y_{j_2,i_1} Z_{j_2,i_1} + 2W_{j_2,j_2} )+ \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2},{\bf 1}_n \rangle 
\end{align*}

where the 1st step from $i_0 = i_1 = i_2$, the 2nd step follows from simple algebra, the 3rd step follows from Lemma~\ref{lem:alpha}, the 4th step follows from Fact~\ref{fac:basic_calculus}, the 5th step follows from Lemma~\ref{lem:gradientUZ}, the 6th step follows from Lemma~\ref{lem:gradientUY_1n}.
\end{proof}
\fi


%\newpage
\subsection{Helpful Lemma for Case 1}

\begin{lemma}[$j_1=j_2$ case]
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
\end{itemize}
We have
\begin{itemize}
    \item {\bf Part 1.} 
    \begin{align*}
        Z_{j_1,i_1}^2 = e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_1}
    \end{align*}
    \item {\bf Part 2.}
    \begin{align*}
            2 Y_{j_1,i_1} Z_{j_1,i_1} = e_{j_1}^\top ( W^\top x_{i_1} x_{i_1}^\top W^\top + W x_{i_1} x_{i_1}^\top W ) e_{j_1}
    \end{align*} 
    \item {\bf Part 3.}
    \begin{align*}
        2 W_{j_1,j_1} = e_{j_1}^\top ( W + W^\top ) e_{j_1}
    \end{align*}
    \item {\bf Part 4.}
    \begin{align*}
        \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1} , {\bf 1}_n \rangle = e_{j_1}^\top ( W^\top X \diag( u(X)_{i_1} ) X^\top W )  e_{j_1}
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}

{\bf Proof Part 1.}

We can show
\begin{align*}
 Z_{j_1,i_1}^2 = & ~ e_{j_1}^\top W x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
    = & ~ e_{j_1}^\top W x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_1}  \\
    = & ~ e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 2.}
On one hand
\begin{align*}
  Y_{j_1, i_1} Z_{j_1, i_1} = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_1} 
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}).

On the other hand
\begin{align*}
  Y_{j_1, i_1} Z_{j_1, i_1} 
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W x_{i_1} \cdot  e_{j_1}^\top W^\top x_{i_1}\\
  = & ~ e_{j_1}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from commutative (Fact~\ref{fac:basic_calculus}), the 3rd step follows from $u^\top v = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}).

{\bf Proof of Part 3.}
It is trivial.

{\bf Proof of Part 4.}
We can show
\begin{align*}
    & ~ \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1} , {\bf 1}_n \rangle\\
    = & ~ \langle u(X)_{i_1} \circ Y_{j_1} , Y_{j_1} \rangle \\
    = & ~ Y_{j_1}^\top (u(X)_{i_1} \circ Y_{j_1}) \\
    = & ~ Y_{j_1}^\top \diag( u(X)_{i_1} )Y_{j_1} \\
    = & ~ e_{j_1}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_1}
\end{align*}

where the 1st step follows from $\langle u \circ v,w\rangle = \langle u \circ v \circ w,{\bf 1}_n \rangle$ (Fact~\ref{fac:basci_algebra}), the 2nd step follows from $v^\top u = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from $u^\top(v \circ w) = u^\top \diag(v)w$ (Fact~\ref{fac:basci_algebra}), the 4th step follows from Definition~\ref{def:Y}.
 

\end{proof}

\begin{lemma}[$j_1\neq j_2$]
 
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
\end{itemize}
We have \Zhao{Your $j_1$ and $j_2$ need to showup both in both sides of the below equation}
\begin{itemize} 
    \item {\bf Part 1.} 
    \begin{align*}
        Z_{j_1,i_1} Z_{j_2,i_1} = e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top ) e_{j_2}
    \end{align*}
    \item {\bf Part 2.}
    \begin{align*}
        Y_{j_1,i_1} Z_{j_2,i_1} = e_{j_1}^\top (W^\top x_{i_1} x_{i_1}^\top W^\top)e_{j_2} 
    \end{align*} 
    \item {\bf Part 3.}
    \begin{align*}
    Y_{j_2, i_1} Z_{j_1, i_1} = e_{j_2}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
    \end{align*}
    \item {\bf Part 4.}
    \begin{align*}
        2 W_{j_2,j_2} = e_{j_2}^\top ( W + W^\top ) e_{j_2}
    \end{align*}
    \item {\bf Part 5.}
    \begin{align*}
        \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2} , {\bf 1}_n \rangle = e_{j_2}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_2} 
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
 

{\bf Proof Part 1.}

We can show
\begin{align*}
Z_{j_1,i_1} Z_{j_2,i_1} = & ~ e_{j_1}^\top W x_{i_1} \cdot e_{j_2}^\top W x_{i_1} \\
 = & ~ e_{j_1}^\top W x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_2} \\
 = & ~ e_{j_1}^\top ( W x_{i_1} x_{i_1}^\top W^\top )  e_{j_2}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 2.}
\begin{align*}
   Y_{j_1,i_1} Z_{j_2,i_1} = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot e_{j_2}^\top W x_{i_1} \\
  = & ~ e_{j_1}^\top W^\top x_{i_1} \cdot x_{i_1}^\top W^\top e_{j_2} \\
  = & ~ e_{j_1}^\top (W^\top x_{i_1} x_{i_1}^\top W^\top)e_{j_2} 
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle = v^\top u$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from Fact~\ref{fac:basic_calculus}.

{\bf Proof Part 3.}
\begin{align*}
  Y_{j_2, i_1} Z_{j_1, i_1} 
  = & ~ e_{j_2}^\top W^\top x_{i_1} \cdot e_{j_1}^\top W x_{i_1} \\
  = & ~ e_{j_2}^\top W x_{i_1} \cdot  e_{j_1}^\top W^\top x_{i_1}\\
  = & ~ e_{j_2}^\top W x_{i_1} x_{i_1}^\top W e_{j_1}
\end{align*}

where the 1st step follows from the Definition~\ref{def:Z} and Definition~\ref{def:Y}, the 2nd step follows from $u^\top v = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra})

{\bf Proof of Part 4.}
It is trivial.

{\bf Proof of Part 5.}
We can show
\begin{align*}
    & ~ \langle u(X)_{i_1} \circ Y_{j_2} \circ Y_{j_2} , {\bf 1}_n \rangle\\
    = & ~ \langle u(X)_{i_1} \circ Y_{j_2} , Y_{j_2} \rangle \\
    = & ~ Y_{j_2}^\top (u(X)_{i_1} \circ Y_{j_2}) \\
    = & ~ Y_{j_2}^\top \diag( u(X)_{i_1} )Y_{j_2} \\
    = & ~ e_{j_2}^\top W^\top X \diag( u(X)_{i_1} ) X^\top W e_{j_2}
\end{align*}

where the 1st step follows from $\langle u \circ v,w\rangle = \langle u \circ v \circ w,{\bf 1}_n \rangle$ (Fact~\ref{fac:basci_algebra}), the 2nd step follows from $v^\top u = \langle u,v \rangle$ (Fact~\ref{fac:basci_algebra}), the 3rd step follows from $u^\top(v \circ w) = u^\top \diag(v)w$ (Fact~\ref{fac:basci_algebra}), the 4th step follows from Definition~\ref{def:Y}.
\end{proof}

\begin{lemma}[Matrix version for Hessian]
If the following conditions hold
\begin{itemize}
    \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
    \begin{align*}
        Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
    \end{align*}
    \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
    \begin{align*}
        Y_{j_1} = X^\top W e_{j_1}
    \end{align*}
    \item Let $Y_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Y},
     \begin{align*}
        Y_{j_1,i_1} = x_{i_1}^\top W e_{j_1}
    \end{align*}
    \item Let 
    \begin{align*}
        H = u(X)_{i_1,i_1} \cdot W x_{i_1} x_{i_1}^\top W^\top + W^\top x_{i_1} x_{i_1}^\top W
    \end{align*}
\end{itemize}
We have
\begin{itemize}
 \item {\bf Part 1.} 
    \begin{align*}
        \frac{ \d \alpha(X)_{i_1} }{ \d x_{i_1,j_1 } \d x_{i_1,j_2} } 
        =  e_{j_1}^\top H e_{j_2}
    \end{align*}
\end{itemize}
\end{lemma}
\begin{proof}
It is obvious by combining Lemma ???,....
\end{proof}

% \subsection{Hessian of Case 2 subblock}

% \begin{lemma}
% If the following conditions
% \begin{itemize}
%     \item $i_0 \neq i_1$, $i_0 = i_2 \in [n]$.
%     \item Let $W = K^\top Q \in \R^{d \times d}$ (for convenient)
%     \begin{itemize}
%         \item For each $j_1, j_2 \in [d]$, we use $W_{j_1,j_2}$ to denote the $(j_1,j_2)$-th entry of $W \in \R^{d \times d}$
%     \end{itemize}
%     \item Let $Z_{j_1,i_1} \in \R$ be defined as Definition~\ref{def:Z}, 
%     \begin{align*}
%         Z_{j_1,i_1} = e_{j_1}^\top W x_{i_1}
%     \end{align*}
%     \item Let $Y_{j_1} \in \R^n$ be defined as Definition~\ref{def:Y},
%     \begin{align*}
%         Y_{j_1} = X^\top W e_{j_1}
%     \end{align*}
% \end{itemize}
% Then we have  
% \begin{itemize}
% \item Part 1.
% \begin{align*}
%     \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} }
%     = & ~ ???u(X)_{i_1,i_1} ( Z_{j_1,i_1}^2 + 2 Y_{j_1,i_1} Z_{j_1,i_1} + 2 W_{j_1,j_1} ) \\
%     & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_1}, {\bf 1}_n \rangle
% \end{align*}
% \item Part 2. $j_1 \neq j_2$  
% \begin{align*}
%      \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_2} }
%     = & ~ ???u(X)_{i_1,i_1} (Z_{j_1, i_1} Z_{j_2,i_1} + Y_{j_1,i_1} Z_{j_2,i_1}+Y_{j_2,i_1} Z_{j_1,i_1} + W_{j_1,j_2}+W_{j_2,j_1} )\\
%     & ~ + \langle u(X)_{i_1} \circ Y_{j_1} \circ Y_{j_2},{\bf 1}_n \rangle 
% \end{align*}
% \end{itemize}
% \end{lemma}
% \begin{proof}
%     \begin{align*}
%         \frac{ \d^2 \alpha(X)_{i_0} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} }
%         = & ~ \frac{ \d^2 \alpha(X)_{i_2} }{ \d x_{i_1,j_1 } \d x_{i_2,j_1} } \\
%         = & ~ \frac{\d }{\d x_{i_1,j_1}} ( \frac{\d \alpha(X)_{i_2} }{\d x_{i_2,j_1}} )
%     \end{align*}
% \end{proof}


\newpage
\Zhao{Don't modify anything after this.}
\subsection{Hessian Split} 
\begin{fact}
Let $H \in \R^{nd \times nd}$ denote the Hessian of $\alpha(X)_{i_0}$, for $i_0 \in [n]$
\begin{align*}
    H = \begin{bmatrix}
        H_{1,1} & H_{1,2} & H_{1,3} & \cdots & H_{1,n} \\
        H_{2,1} & H_{2,2} & H_{2,3} & \cdots & H_{2,n} \\
        H_{3,1} & H_{3,2} & H_{3,3} & \cdots & H_{3,n} \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        H_{n,1} & H_{n,2} & H_{n,3} & \cdots & H_{n,n}
    \end{bmatrix}
\end{align*}
where $H_{i_1,i_2} \in \R^{d \times d}$ for each $i_1,i_2 \in [n]$ and each entry of  $H_{i_1,i_2}$ can written as
\begin{align*}
    (H_{i_1,i_2})_{j_1,j_2} = \frac{\d^2 \alpha(X)_{i_0}}{\d x_{i_1,j_1} \d x_{i_2,j_2}}, \forall j_1, j_2 \in [d]
\end{align*}

\end{fact}

\Zhao{The real version you care is}
\begin{align*}
    (H_{i_1,i_2})_{j_1,j_2} = \frac{\d^2 c(X)_{i_0,j_0}}{\d x_{i_1,j_1} \d x_{i_2,j_2}}, \forall j_1, j_2 \in [d]
\end{align*}

Imagine if the claim is for DLS23, 
\begin{claim}
The cases we care are 
\begin{itemize}
    \item Case 1. $i = j$
    \item Case 2. $i \neq j$
\end{itemize}
\end{claim}
 
\begin{claim}
For $i_0$ is fixed, there 5 subblocks $H_{i_1,i_2}$ we need to care
\begin{itemize}
    \item Case 1. $i_0 = i_1 = i_2$
    \item Case 2. $i_0 \neq i_1$, $i_0 = i_2$
    \item Case 3. $i_0 = i_1 $, $i_0 \neq i_2$
    \item Case 4. $i_0 \neq i_1$, $i_0 \neq i_2$, $i_1 = i_2$
    \item Case 5. $i_0 \neq i_1 $, $i_0 \neq i_2$, $i_1 \neq i_2$
\end{itemize}
\end{claim}

\begin{fact}
Suppose $i_0 = 1$,\Yichuan{What are these $C$'s?} \Zhao{$C1$ means Case 1.}
\begin{align*}
    H = \begin{bmatrix}
        C1 & C3 & C3 & \cdots & C3 \\
        C2 & C4 & C5 & \cdots & C5 \\
        C2 & C5 & C4 & \cdots & C5 \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        C2 & C5 & C5 & \cdots & C4
    \end{bmatrix}
\end{align*}
\end{fact}


\begin{fact}
Suppose $i_0 = 2$,
\begin{align*}
    H = \begin{bmatrix}
        C4 & C2 & C5 & \cdots & C5 \\
        C3 & C1 & C3 & \cdots & C3 \\
        C5 & C2 & C5 & \cdots & C5 \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        C5 & C2 & C5 & \cdots & C5
    \end{bmatrix}
\end{align*}
\end{fact}

\begin{fact}
Suppose $i_0 = 3$,
\begin{align*}
    H = \begin{bmatrix}
        C4 & C5 & C2 & \cdots & C5 \\
        C5 & C4 & C2 & \cdots & C5 \\
        C3 & C3 & C1 & \cdots & C3 \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        C5 & C5 & C2 & \cdots & C4
    \end{bmatrix}
\end{align*}
\end{fact}

\begin{fact}
Suppose $i_0 = n$,
\begin{align*}
    H = \begin{bmatrix}
        C4 & C5 & C5 & \cdots & C2 \\
        C5 & C4 & C5 & \cdots & C2 \\
        C5 & C5 & C4 & \cdots & C2 \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        C3 & C3 & C3 & \cdots & C1
    \end{bmatrix}
\end{align*}
\end{fact}



==> hessian_more.tex <==

\section{Hessian more}
%\newpage
\subsection{Hessian of \texorpdfstring{$\alpha(X)^{-1}_{i_1}$}{}}
\begin{lemma}[A generalization of Lemma 5.11 in \cite{dls23}]
If the following conditions hold
\begin{itemize}
    \item Let $Q \in \R^{d \times d}$.
    \item Let $K \in \R^{d \times d}$.
    \item Let $X \in \R^{d \times n}$.
    \item Let $\alpha(X)$ be defined as Definition $\ref{def:alpha}$
    \item Let $Z_{i_1,j_1,i_1}$ be defined as Definition $\ref{def:Z}$
    \item Let $Y_{i_1,j_1}$ be defined as Definition $\ref{def:Y}$ 
    \item Let $e_i$ denote a vector only $i$-th entry is $1$ and zero everywhere else.
    \item Let ${\bf 1}_n$ denote a length-$n$ vector where all the entries are ones.
\end{itemize}
Then we have 
\begin{itemize}
     \item Part 1.
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_1}} \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ - ({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 \\
        & ~ + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle 
    \end{align*}
    \item Part 2. 
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_2}} \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot \langle  u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})  
         \\
        & ~ + u(X)_{i_1} \circ (( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} )+({ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}), {\bf 1}_n \rangle  
    \end{align*}
    \item Part 3. Let $i_2 \neq i_1$. 
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{ \d x_{i_1,j_1} \d x_{i_2,j_2} } \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-}({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle
    \end{align*}
    \item Part 4. Let $i_1 \neq i_2$
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{  \d x_{i_2,j_2} \d x_{i_2,j_2} } \\ 
        = & ~  {-2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle ^{2} \\
        & ~ + {-}{\alpha(X)_{i_1} } ^{-2} \cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})   \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle
    \end{align*}
    \item Part 5. Let $i_1 \neq i_2$, let $j_2 \neq j_3$
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)_{i_1}^{-1} }{  \d x_{i_2,j_2} \d x_{i_2,j_3} } \\ 
        = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \\
        & ~ - {\alpha(X)_{i_1} } ^{-2} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle 
    \end{align*}
    \item Part 6. Let $i_1 \neq i_2 \neq i_3$
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{  \d x_{i_2,j_2} \d x_{i_3,j_3} }\\
        = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ Z_{i_3,j_3,i_1} , {\bf 1}_n  \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_3,j_3,i_1} , {\bf 1}_n  \rangle 
    \end{align*}
\end{itemize}
\begin{proof}
    {\bf Proof of Part 1.}
\begin{align}\label{eq:d_u_Z_Y_1_n_d_x}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}} \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \notag \\
    = & ~  \langle \frac{ \d}{ \d x_{i_1, j_1}} (u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), \frac{ \d}{ \d x_{i_1, j_1}} {\bf 1}_n \rangle \notag \\
    = & ~ \langle u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), \frac{ \d}{ \d x_{i_1, j_1}} {\bf 1}_n \rangle \notag \\
    = & ~ \langle u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 0}_n \rangle \notag \\
    = & ~ \langle u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle 
\end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:gradU(YZ)}, 
the 3th step follows from simple algebra, the 4th step follows from simple algebra.

\begin{align*}
        & ~  \frac{ \d^2 \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_1}} \\
        = & ~  \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_1}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle  \\
        = & ~ {-} (\frac{ \d}{ \d x_{i_1, j_1}} ({\alpha(X)_{i_1} }) ^{-2}) \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ - ({\alpha(X)_{i_1} }) ^{-2}) \cdot  \frac{ \d}{ \d x_{i_1, j_1}} \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ - ({\alpha(X)_{i_1} }) ^{-2} \cdot  \frac{ \d}{ \d x_{i_1, j_1}} \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ - ({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 \\
        & ~ + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle 
    \end{align*}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, 
the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from Eq.~\eqref{eq:d_u_Z_Y_1_n_d_x}, the 5th step follows from simple algebra.

{\bf Proof of Part 2.}
\begin{align}\label{eq:d_u_Z_Y_2_n_d_x}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}} \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle \notag \\
    = & ~  \langle \frac{ \d}{ \d x_{i_1, j_1}} (u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), \frac{ \d}{ \d x_{i_1, j_1}} {\bf 1}_n \rangle \notag \\
    = & ~ \langle  u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})  
    \notag \\
    & ~ + u(X)_{i_1} \circ (( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} )+({ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), \frac{ \d}{ \d x_{i_1, j_1}} {\bf 1}_n \rangle \notag \\
    = & ~ \langle  u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})  
    \notag \\
    & ~ + u(X)_{i_1} \circ (( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} )+({ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}), {\bf 1}_n \rangle \notag \\
    & ~ + \langle    u(X)_{i_1} \circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 0}_n \rangle \notag \\
    = & ~ \langle  u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})  
    \notag \\
    & ~ + u(X)_{i_1} \circ (( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} )+({ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}), {\bf 1}_n \rangle 
\end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:gradU(YZ)}, 
the 3th step follows from simple algebra, the 4th step follows from simple algebra.

    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_2}} \\
         = & ~  \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_1, j_2}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle  \\
        = & ~  {-} (\frac{ \d}{ \d x_{i_1, j_1}}({\alpha(X)_{i_1} }) ^{-2}) \cdot  \langle    u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle  \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot \frac{ \d}{ \d x_{i_1, j_1}} \langle   ( u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle) \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot \frac{ \d}{ \d x_{i_1, j_1}} \langle   ( u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle) \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2} \cdot \langle  u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2})  
         \\
        & ~ + u(X)_{i_1} \circ (( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} )+({ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}), {\bf 1}_n \rangle  
    \end{align*}

where the 1st step follows from simple algebra, the 2nd step follows from 
Fact~\ref{fac:basic_calculus}, the 3rd step follows from the Lemma~\ref{lem:alpha^-2}, 
the 4th step follows from Fact~\ref{fac:basic_calculus}, the 5th step follows from Eq.~\eqref{eq:d_u_Z_Y_2_n_d_x}, the 5th step follows from simple algebra.

{\bf Proof of Part 3.}

\begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{ \d x_{i_1,j_1} \d x_{i_2,j_2} } \\
        = & ~  \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_2, j_2}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} ({-}({\alpha(X)_{i_1} }) ^{-2} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) \\
        = & ~ (\frac{ \d}{ \d x_{i_1, j_1}} {-}({\alpha(X)_{i_1} }) ^{-2} )\cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) \\
        & ~ {-}({\alpha(X)_{i_1} }) ^{-2} \cdot  \frac{ \d}{ \d x_{i_1, j_1}} (\langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) \\
        = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-}({\alpha(X)_{i_1} }) ^{-2} \cdot  \frac{ \d}{ \d x_{i_1, j_1}} (\langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) \\
         = & ~ {2} \cdot ({\alpha(X)_{i_1} }) ^{-3}\cdot 
        \langle   u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ {-}({\alpha(X)_{i_1} }) ^{-2} \cdot  \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle
    \end{align*}
    
where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from the Lemma~\ref{lem:alpha^-2}, the 5th step follows from Lemma~\ref{lem:gradUZ}.

{\bf Proof of Part 4.}
    \begin{align*}
        & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{  \d x_{i_2,j_2} \d x_{i_2,j_2} }\\
        = & ~ \frac{ \d}{ \d x_{i_2, j_2}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_2, j_2}})\\
        = & ~ \frac{ \d}{ \d x_{i_2, j_2}}
        ({-}{\alpha(X)_{i_1} }) ^{-2} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) \\
        = & ~ \frac{ \d}{ \d x_{i_2, j_2}}
        ({-}{\alpha(X)_{i_1} }) ^{-2}) \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \\
        & ~ + {-}{\alpha(X)_{i_1} } ^{-2} \cdot \frac{ \d}{ \d x_{i_2, j_2}}(\langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle)\\
        = & ~  {-2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \\
        & ~ + {-}{\alpha(X)_{i_1} } ^{-2} \cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \\
        & ~ \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \\
        = & ~  {-2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle ^{2} \\
        & ~ + {-}{\alpha(X)_{i_1} } ^{-2} \cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \\
        & ~ \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle
    \end{align*}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from the Lemma~\ref{lem:alpha^-2}, the 5th step follows from Lemma~\ref{lem:gradUZ}.

{\bf Proof of Part 5.}
    
    \begin{align}\label{eq:u_Z_2_3_1n_d_x}
        & ~ \frac{ \d}{ \d x_{i_2, j_2}}\langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \notag \\
        = & ~ \langle \frac{ \d}{ \d x_{i_2, j_2}}(u(X)_{i_1} \circ Z_{i_2,j_3,i_1}) , {\bf 1}_n  \rangle \notag \\
        & ~ + \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , \frac{ \d}{ \d x_{i_2, j_2}}({\bf 1}_n)  \rangle \notag \\
        = & ~ \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \notag \\
        & ~ + \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , \frac{ \d}{ \d x_{i_2, j_2}}({\bf 1}_n)  \rangle \notag \\
        = & ~ \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \notag \\
        & ~ + \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} ,({\bf 0}_n)  \rangle \notag \\
        = & ~ \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle 
    \end{align}
    
where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:gradUZ}, the 3rd step follows from simple algebra, the 4th step follows from the simple algebra.
    
    \begin{align*}
    & ~ \frac{ \d^2 \alpha(X)_{i_1}^{-1} }{  \d x_{i_2,j_2} \d x_{i_2,j_3} } \\ 
    = & ~ \frac{ \d}{ \d x_{i_2, j_2}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_2, j_3}})\\
    = & ~ \frac{ \d}{ \d x_{i_2, j_2}} ({-}({\alpha(X)_{i_1} }) ^{-2} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle)\\
    = & ~ (\frac{ \d}{ \d x_{i_2, j_2}} {-}({\alpha(X)_{i_1} }) ^{-2}) \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \\
    & ~ - {\alpha(X)_{i_1} } ^{-2} \cdot \frac{ \d}{ \d x_{i_2, j_2}}(\langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle) \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \\
    & ~ - {\alpha(X)_{i_1} } ^{-2} \cdot \frac{ \d}{ \d x_{i_2, j_2}}(\langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle) \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle \\
    & ~ - {\alpha(X)_{i_1} } ^{-2} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_2,j_3,i_1} , {\bf 1}_n  \rangle 
    \end{align*}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from Lemma~\ref{lem:alpha^-2}, the 5th step follows from Eq.~\eqref{eq:u_Z_2_3_1n_d_x}.

{\bf Proof of Part 6.}
\begin{align}\label{eq:u_Z_2_2_1n_d_x}
    & ~ \frac{ \d}{ \d x_{i_2, j_2}} u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) \notag \\
    = & ~ \frac{ \d}{ \d x_{i_2, j_2}}(u(X)_{i_1}) \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})\notag \\
    & ~ + u(X)_{i_1} \circ \frac{ \d}{ \d x_{i_2, j_2}}(e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})\notag \\
    = & ~ u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})\notag \\
    & ~ + u(X)_{i_1} \circ \frac{ \d}{ \d x_{i_2, j_2}}(e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})\notag \\
    = & ~ u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})\notag \\
    & ~ + u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q {\bf 0}_d)\notag \\
    = & ~ u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})
\end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:gradUX}, the 3rd step follows from simple algebra, the 4th step follows from simple algebra.

\begin{align*}
    & ~ \frac{ \d^2 \alpha(X)^{-1}_{i_1} }{  \d x_{i_2,j_2} \d x_{i_3,j_3} } \\
    = & ~ \frac{ \d}{ \d x_{i_2, j_2}} (\frac{ \d \alpha(X)^{-1}_{i_1} } { \d x_{i_3, j_3}})\\
    = & ~ \frac{ \d}{ \d x_{i_2, j_2}} ({-} ({\alpha(X)_{i_1} }) ^{-2} \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle )\\
    = & ~  ({-} \frac{ \d}{ \d x_{i_2, j_2}}({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \frac{ \d}{ \d x_{i_2, j_2}}(\langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle) \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \frac{ \d}{ \d x_{i_2, j_2}}(\langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle) \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  \frac{ \d}{ \d x_{i_2, j_2}}(u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1})) , {\bf 1}_n  \rangle \\
    & ~ + \langle u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , \frac{ \d}{ \d x_{i_2, j_2}}( {\bf 1}_n ) \rangle  \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ + \langle u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , \frac{ \d}{ \d x_{i_2, j_2}}( {\bf 1}_n ) \rangle  \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ + \langle u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , \frac{ \d}{ \d x_{i_2, j_2}}( {\bf 0}_n ) \rangle  \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ (e_{i_3} e_{j_3}^\top K^\top Q x_{i_1}) , {\bf 1}_n  \rangle \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-3}  \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \cdot \langle  u(X)_{i_1} \circ Z_{i_3,j_3,i_1} , {\bf 1}_n  \rangle \\
    & ~ {-} ({\alpha(X)_{i_1} } ^{-2}) \cdot \langle  u(X)_{i_1} \circ Z_{i_2,j_2,i_1} \circ Z_{i_3,j_3,i_1}  , {\bf 1}_n  \rangle 
\end{align*}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from Lemma~\ref{lem:alpha^-2}, the 5th step follows from Fact~\ref{fac:basic_calculus}, the 6th step follows from Eq.\eqref{eq:u_Z_2_2_1n_d_x}, the 7th step follows from simple algebra, the 8th step follows from simple algebra.
\end{proof}
\end{lemma}


\subsection{Hessian of \texorpdfstring{$f(X)$}{}}
\begin{lemma}[A generalization of Lemma 5.12 in \cite{dls23}]
If the following conditions hold
\begin{itemize}
    \item Let $Q \in \R^{d \times d}$.
    \item Let $K \in \R^{d \times d}$.
    \item Let $X \in \R^{d \times n}$.
     \item Let $f(X)$ be defined as Definition $\ref{def:f}$
     \item Let $\alpha(X)$ be defined as Definition $\ref{def:alpha}$
    \item Let $Z_{i_1,j_1,i_1}$ be defined as Definition $\ref{def:Z}$
    \item Let $Y_{i_1,j_1}$ be defined as Definition $\ref{def:Y}$ 
    \item Let $e_i$ denote a vector only $i$-th entry is $1$ and zero everywhere else.
    \item Let ${\bf 1}_n$ denote a length-$n$ vector where all the entries are ones.
\end{itemize}
Then we have 
\begin{itemize}
\item Part 1.
\begin{align*}
     & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_1}} \\
     = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \\
        & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n\rangle \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ Y_{i_1,j_1} + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}) \\
\end{align*}
\item Part 2.
\begin{align*}
        & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_2}} \\
        = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag\\
         & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}) \notag\\
        & ~ + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}+e_{i_1} e_{j_1}^\top K^\top Qe_{j_2}) \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}), {\bf 1}_n\rangle \\
        & ~ + f(X)_{i_1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2})  
        \\
         & ~ + u(X)_{i_1} \circ ( e_{i_1} e_{j_2}^\top K^\top Q  e_{j_1} +{ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}) 
 \end{align*}
 \item Part 3.
\begin{align*}
    & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_1, j_1} \d x_{i_2,j_2}} \\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \\
    & ~ -\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \circ Z_{i_2,j_2,i_1}\\
    & ~ + f(X)_{i_1}  \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} 
\end{align*}
 \item Part 4.
 \begin{align*}
 & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_2, j_2} \d x_{i_2,j_2}} \\
 \end{align*}
  \item Part 5.
 \begin{align*}
 & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_2, j_2} \d x_{i_2,j_3}} \\
 \end{align*}
   \item Part 6.
 \begin{align*}
 & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_2, j_2} \d x_{i_3,j_3}} \\
 \end{align*}
\end{itemize}
\begin{proof}
    {\bf Proof of Part 1.}
    \begin{align}\label{eq:alpha_f_u_Z_Y}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \notag\\
    = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}(\langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle)) \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}\langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle
    \end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha_-1_f}, the 3rd step follows from Lemma~\ref{lem:gradU(YZ)}.

    \begin{align}\label{eq:d_alpha_u_Z_Y}
        & ~ \frac{ \d}{ \d x_{i_1, j_1}}(\alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))) \notag \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(\alpha(X)_{i_1}^{-1}) \cdot (u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))  \notag \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot \frac{ \d}{ \d x_{i_1, j_1}}(u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag \\
        = & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n\rangle \notag \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot \frac{ \d}{ \d x_{i_1, j_1}}(u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag \\
        = & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n\rangle \notag \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ Y_{i_1,j_1} + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}) \notag \\
    \end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha^-1}, the 3rd step follows from Lemma~\ref{lem:gradU(YZ)}.

    \begin{align*}
        & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_1}} \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d f(X)_{i_1} } { \d x_{i_1, j_1}}) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))) \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \\
        & ~ + \frac{ \d}{ \d x_{i_1, j_1}}(\alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))) \\
        = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \\
        & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle \\
        & ~ + \frac{ \d}{ \d x_{i_1, j_1}}(\alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1}\circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))) \\
        = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}))\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle) \\
        & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ ((Z_{i_1,j_1,i_1}+Y_{i_1,j_1})^2 + 2 \cdot ( e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1} ) ), {\bf 1}_n \rangle \\
        & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n\rangle \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ Y_{i_1,j_1} + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}) \\
    \end{align*}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from Lemma~\ref{lem:f(x)}, the 3rd step follows from the Fact~\ref{fac:basic_calculus}, the 4th step follows from Eq.~\eqref{eq:alpha_f_u_Z_Y}, the 5th step follows from Eq.~\eqref{eq:d_alpha_u_Z_Y}

    {\bf Proof of Part 2.}
    \begin{align}\label{eq:alpha_f_u12_Z_Y}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle) \notag\\
    = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}(\langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle)) \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag\\
     & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}(\langle ( u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}), {\bf 1}_n \rangle)) \notag\\
     = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag\\
     & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}) \notag\\
     & ~ + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}+e_{i_1} e_{j_1}^\top K^\top Qe_{j_2}) 
    \end{align}


where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from Lemma~\ref{lem:alpha_-1_f}, the 3rd step follows from the Fact~\ref{fac:basic_calculus}, the 3rd step follows from Lemma~\ref{lem:gradU(YZ)}.
    
    \begin{align}\label{eq:d_alpha_u12_Z_Y}
        & ~ \frac{ \d}{ \d x_{i_1, j_1}}(f(X)_{i_1} \cdot (u(X)_{i_1}\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}))) \notag \\
        = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(f(X)_{i_1}) \cdot (u(X)_{i_1}\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}))  \notag \\
        & ~ + f(X)_{i_1} \cdot \frac{ \d}{ \d x_{i_1, j_1}}(u(X)_{i_1}\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2})) \notag \\
        = & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}), {\bf 1}_n\rangle \notag \\
        & ~ + f(X)_{i_1} \cdot \frac{ \d}{ \d x_{i_1, j_1}}(u(X)_{i_1}\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2})) \notag \\
        = & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}), {\bf 1}_n\rangle \notag \\
        & ~ + f(X)_{i_1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2})  
    \notag \\
    & ~ + u(X)_{i_1} \circ ( e_{i_1} e_{j_2}^\top K^\top Q  e_{j_1} +{ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2})  \notag \\
    \end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:f(x)}, the 3rd step follows from Lemma~\ref{lem:gradU(YZ)}.
    
    \begin{align*}
     & ~ \frac{ \d^2 f(X)_{i_1} } { \d x_{i_1, j_1} \d x_{i_1,j_2}} \\
     = & ~ \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d f(X)_{i_1} } { \d x_{i_1, j_2}}) \\
     = & ~ \frac{ \d}{ \d x_{i_1, j_1}}({-} ({\alpha(X)_{i_1} }) ^{-1} \cdot f(X)_{i_1} \circ \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1} + Y_{i_1,j_2}), { \bf 1}_n \rangle \\
     & ~ + f(X)_{i_1} \circ (Z_{i_1,j_2,i_1} + Y_{i_1,j_2}) \\
     = & ~ \frac{ \d}{ \d x_{i_1, j_1}}({-} ({\alpha(X)_{i_1} }) ^{-1} \cdot f(X)_{i_1} \cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1} + Y_{i_1,j_2}), { \bf 1}_n \rangle) \\
     & ~ + \frac{ \d}{ \d x_{i_1, j_1}}(f(X)_{i_1} \circ (Z_{i_1,j_2,i_1} + Y_{i_1,j_2}) \\
     = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag\\
     & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}) \notag\\
     & ~ + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}+e_{i_1} e_{j_1}^\top K^\top Qe_{j_2}) \\
      & ~ + \frac{ \d}{ \d x_{i_1, j_1}}(f(X)_{i_1} \circ (Z_{i_1,j_2,i_1} + Y_{i_1,j_2}) \\
      = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag\\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \notag\\
     & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_2}) \notag\\
     & ~ + u(X)_{i_1} \circ (e_{i_1} e_{j_1}^\top K^\top Q  e_{j_1}+e_{i_1} e_{j_1}^\top K^\top Qe_{j_2}) \\
    & ~ {-} ({\alpha(X)_{i_1} }) ^{-2}\cdot  \langle u(X)_{i_1} \circ 
        (Z_{i_1,j_2,i_1}+Y_{i_1,j_2}), {\bf 1}_n\rangle \\
        & ~ + f(X)_{i_1} \cdot u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})\circ (Z_{i_1,j_2,i_1}+Y_{i_1,j_2})  
    \\
    & ~ + u(X)_{i_1} \circ ( e_{i_1} e_{j_2}^\top K^\top Q  e_{j_1} +{ e_{i_1} }e_{j_1}^\top K^\top Q e_{j_2}) 
    \end{align*}
    
where the 1st step follows from simple algebra, the 2nd step follows from simple algebra, the 3rd step follows from Fact~\ref{fac:basic_calculus}, the 4th step follows from Eq.~\eqref{eq:alpha_f_u12_Z_Y}, the 5th step follows from Eq.~\eqref{eq:d_alpha_u12_Z_Y}.

    {\bf Proof of Part 3.}
    \begin{align}\label{eq:d_alpha_f_Z_221}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}}({-}({\alpha(X)_{i_1} }) ^{-1} f(X)_{i_1} \cdot \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle \notag \\
    = & ~ \frac{ \d}{ \d x_{i_1, j_1}}(-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}(\langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \frac{ \d}{ \d x_{i_1, j_1}}(\langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \notag\\
    = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \notag \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \notag\\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \notag\\
    \end{align}
    
where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:alpha_-1_f}, the 3rd step follows from Lemma~\ref{lem:gradU(YZ)}.

\begin{align}\label{eq:d_f_Z_221}
    & ~ \frac{ \d}{ \d x_{i_1, j_1}} (f(X)_{i_1}  \circ Z_{i_2,j_2,i_1}) \notag \\
    = & ~ \frac{ \d}{ \d x_{i_1, j_1}} (f(X)_{i_1})  \circ Z_{i_2,j_2,i_1} \notag \\
    & ~ + f(X)_{i_1}  \circ \frac{ \d}{ \d x_{i_1, j_1}}(Z_{i_2,j_2,i_1}) \notag \\
    = & ~ -\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \notag \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \circ Z_{i_2,j_2,i_1} \notag \\
    & ~ + f(X)_{i_1}  \circ \frac{ \d}{ \d x_{i_1, j_1}}(Z_{i_2,j_2,i_1}) \notag \\
    = & ~ -\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \notag \\
        & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \circ Z_{i_2,j_2,i_1} \notag \\
    & ~ + f(X)_{i_1}  \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1}  \notag \\
\end{align}

where the 1st step follows from
Fact~\ref{fac:basic_calculus}, the 2nd step follows from the Lemma~\ref{lem:f(x)}, the 3rd step follows from Lemma~\ref{lem:Z}.

    \begin{align*}
     & ~ \frac{ \d}{ \d x_{i_1, j_1}} (\frac{ \d f(X)_{i_1} } { \d x_{i_2, j_2}}) \\
     = & ~ \frac{ \d}{ \d x_{i_1, j_1}}({-}({\alpha(X)_{i_1} }) ^{-1} \cdot f(X)_{i_1} \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle + f(X)_{i_1}  \circ Z_{i_2,j_2,i_1}) \\
     = & ~ \frac{ \d}{ \d x_{i_1, j_1}}({-}({\alpha(X)_{i_1} }) ^{-1} \cdot f(X)_{i_1} \langle u(X)_{i_1} \circ Z_{i_2,j_2,i_1} , {\bf 1}_n \rangle) +\frac{ \d}{ \d x_{i_1, j_1}}( f(X)_{i_1}  \circ Z_{i_2,j_2,i_1}) \\
     = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \\
    & ~ + \frac{ \d}{ \d x_{i_1, j_1}}( f(X)_{i_1}  \circ Z_{i_2,j_2,i_1}) \\
     = & ~ {2} \cdot (\alpha(X)_{i_1} ) ^{-2}\cdot  \langle u(X)_{i_1}\circ 
    (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle f(X)_{i_1} \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \cdot \langle ( u(X)_{i_1} \circ Z_{i_2,j_2,i_1}), {\bf 1}_n \rangle) \\
    & ~ + (-\alpha(X)_{i_1}^{-1} f(X)_{i_1})\cdot \langle u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1}) \circ Z_{i_2,j_2,i_1}+ u(X)_{i_1} \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} , {\bf 1}_n \rangle \\
    & ~ -\alpha(X)_{i_1}^{-1} f(X)_{i_1}\cdot \langle ( u(X)_{i_1} \circ Z_{i_1,j_1,i_1}+Y_{i_1,j_1}), {\bf 1}_n \rangle \\
    & ~ + \alpha(X)_{i_1}^{-1} \cdot (u(X)_{i_1} \circ (Z_{i_1,j_1,i_1}+Y_{i_1,j_1})) \circ Z_{i_2,j_2,i_1}\\
    & ~ + f(X)_{i_1}  \circ e_{i_2} e_{j_2}^\top K^\top Q  e_{j_1} 
    \end{align*}

where the 1st step follows from Lemma~\ref{lem:f(x)}, the 2nd step follows from Fact~\ref{fac:basic_calculus}, the 3rd step follows from the Eq.~\eqref{eq:d_alpha_f_Z_221}, the 4th step follows from Eq.~\eqref{eq:d_f_Z_221}.
    \end{proof}
\end{lemma}

\begin{table}[!ht]\caption{Summary of Hessian}

\begin{center}
\begin{tabular}{ |l|l|l|l|l|l| } \hline
 Notations(\cite{dls23}) & Parts & Dim & Notation(Ours) & Parts & Dim \\ \hline
 $\exp(Ax)$ & 2 Parts & $\R^n$ & $u_{i_1}(x)$ &6 Parts& $\R^n$ \\ \hline
$\alpha(x)$ & 2 Parts &$\mathrm{scalar}$ & $\alpha(x)_{i_1}$ & 6 Parts & $\mathrm{scalar}$ \\  \hline
$\alpha(x)^{-1}$ & 2 Parts & $\mathrm{scalar}$ & $\alpha(x)_{i_1}^{-1}$ & 6 Parts & $\mathrm{scalar}$ \\  \hline
$f(x)$ & 2 Parts & $\R^n$ & $f(x)_{i_1}$ & 6 Parts& $\R^n$  \\  \hline
$L(x)$ & 2 Parts &  $\mathrm{scalar}$ & $L(x)$ & 6 Parts & $\mathrm{scalar}$ \\ \hline
\end{tabular}
\end{center}

\end{table}

\subsection{Hessian of \texorpdfstring{$L(X)$}{}}
\begin{lemma}[A generalization of Lemma 5.13 in \cite{dls23}]
If the following conditions hold
\begin{itemize}
    \item Let $Q \in \R^{d \times d}$.
    \item Let $K \in \R^{d \times d}$.
    \item Let $V \in \R^{d \times d}$.
    \item Let $X \in \R^{d \times n}$.
    \item Let $L(X)$ be defined as Definition $\ref{def:L}$.
    \item Let $A(X)$ be defined as Definition $\ref{def:L}$.
    \item Let $D(X)$ be defined as Definition $\ref{def:L}$.
    \end{itemize}
    Then, we have
\begin{itemize}
    \item {\bf Part 1.}  Let $i_1 \in [n]$, $j_1 \in [d]$
    \begin{align*}
    \frac{\d^2 L(x)}{\d x_{i_1,j_1} \d x_{i_1,j_1}}
    \end{align*}
    \end{itemize}
\iffalse
\begin{align*}
    L( X ) = & ~ 0.5 \cdot \| D(X)^{-1}  A(X) X^\top  V - B\|_F^2 \\
    = & ~ 0.5 \cdot Tr[(D(X)^{-1}  A(X) X^\top  V - B)(D(X)^{-1}  A(X) X^\top  V - B)^\top] \\
    = & ~ 0.5 \cdot 
    Tr[(D(X)^{-1}  A(X) X^\top  V)(D(X)^{-1}  A(X) X^\top  V )^\top \\ 
    & ~ - (D(X)^{-1} A(X) X^\top  V) \cdot B^\top-B \cdot (D(X)^{-1} A(X) X^\top  V)^\top+B \cdot B^\top] \\
    = & ~ 0.5 \cdot 
    Tr[I - (D(X)^{-1} A(X) X^\top  V) \cdot B^\top-B \cdot (D(X)^{-1} A(X) X^\top  V)^\top + I] \\
    = & ~ 0.5 \cdot \mathrm Tr[I]-Tr[(D(X)^{-1} A(X) X^\top  V)]-Tr[B \cdot (D(X)^{-1} A(X) X^\top  V)^\top]+Tr[I]
\end{align*}
\fi
\iffalse
\begin{align*}
    & ~ \frac{ \d}{ \d X} Tr[(D(X)^{-1} A(X) X^\top  V)] \\
    = & ~ \frac{ \d}{ \d x_{i_1, j_1}} Tr[(D(X)^{-1} A(X) X^\top  V)] \\
    = & ~ \Sigma_{i}
\end{align*}
\begin{align*}
    \nabla L(X) = 
\end{align*}
\begin{align*}
    A(X) = \exp( X^\top Q^\top K^\top X) \\
    D(X) = \diag( A(X) {\bf 1}_n ) \\
    d D = \diag ({\bf 1}_n \cdot d A(X))\\
    =  \diag ({\bf 1}_n \cdot d A(X))
    \end{align*}
    \begin{align*}
    L(X + \Delta X) = \\
    Z = D A X^\top \\
    dZ = d(D A X^\top)
\end{align*}
\fi
\end{lemma}


==> lipschitz.tex <==
\section{Lipschitz}

\subsection{Hessian is Lipschitz}

\subsection{Lipschitz Property for Several Basic Functions}
\begin{lemma}
If the following conditions hold
\begin{itemize}
    \item Let $A \in \R^{n \times d}$.
    \item Let $Q \in \R^{d \times d}$.
    \item Let $K \in \R^{d \times d}$.
    \item Let $X \in \R^{d \times n}$.
     \item Let $f(X)$ be defined as Definition $\ref{def:f}$
     \item Let $\alpha(X)$ be defined as Definition $\ref{def:alpha}$
     \item Let $f(X)$ be defined as Definition $\ref{def:f}$
    \item Let $Z_{i_1,j_1,i_1}$ be defined as Definition $\ref{def:Z}$
    \item Let $Y_{i_1,j_1}$ be defined as Definition $\ref{def:Y}$ 
    \item Let $e_i$ denote a vector only $i$-th entry is $1$ and zero everywhere else.
    \item Let ${\bf 1}_n$ denote a length-$n$ vector where all the entries are ones.
\end{itemize}
Then we have 
\begin{itemize}
\item Part 0.
\begin{align*}
\lVert u(X) \rVert
\end{align*}
\item Part 1.
\begin{align*}
\lVert u(X)-u(Y) \rVert
\end{align*}
\item Part 2.
\begin{align*}
|\alpha(X)-\alpha(Y)| \leqslant K \lVert u(X)-u(Y) \rVert_{2}
\end{align*}
\item Part 3.
\begin{align*}
|\alpha(X)^{-1}-\alpha(Y)^{-1}| \leqslant L | \alpha(X)-\alpha(Y)|
\end{align*}
\item Part 3.
\begin{align*}
\lVert f(X)-f(Y) \rVert_{2}
\end{align*}
\end{itemize}
\end{lemma}

==> tech_ov.tex <==
\section{Technique Overview}
Here in this section, we provide an overview of our techniques. 

\paragraph{Inverting the Attention with Hessian and Weights.}
In this work, we propose a novel technique for inverting the attention weights of a transformer model using Hessian decomposition. Specifically, given the attention weights $W = KQ^\top \in \mathbb{R}^{d \times d}$, output $B \in \mathbb{R}^{n \times d}$, and diagonal matrix $D(X) = \diag(\exp(X^\top W X)) \in \mathbb{R}^{n \times n}$, we aim to find the input $X \in \mathbb{R}^{d \times n}$ that minimizes the Frobenius norm of the difference between $D(X)^{-1} \text{exp}(X^\top W X) V - B$, where $V \in \mathbb{R}^{d \times d}$ is a matrix of values. To achieve this, we introduce an algorithm that minimizes the loss function $L(X)$, defined as
\begin{align}
\label{eq:loss}
    L(X):=\| \underbrace{D(X)^{-1} \exp( X^\top W X ) }_{n \times n} \underbrace{X^\top}_{n \times d} \underbrace{V}_{d \times d} - \underbrace{B}_{n \times d} \|_F^2,
\end{align}
which captures the discrepancy between the expected output and the actual output of the transformer. Our approach leverages Hessian decomposition to efficiently compute the Hessian and to apply second-order method to approximate the optimal input of $X$. \Yichuan{Maybe add more details when the main result is finished}

\paragraph{Hessian Decomposition.}
Due to the complexity of the loss function (Eq.\eqref{eq:loss}), it is difficult (or basically impossible) to compute its Hessian directly. In order to simplify this, we define several notations, 
\begin{align*}
    \text{Exponential Function:}~ u(X)_i & := \exp(X^\top W X_{*,i}) \\
    \text{Sum of Softmax:}~ \alpha(X)_i & := \langle u(X)_i, \mathbf{1}_n \rangle \\
    \text{Softmax Probability:}~ f(X)_i & := \alpha(X)_i^{-1}u(X)_i \\
    \text{Value Function:}~ h(X)_j &:= X^\top V_{*, j} \\
    \text{One-unit Loss Function:}~ c(X)_{i,j} &:= \langle f(X)_i, h(X)_j \rangle - b_{i,j}.
\end{align*}
Using these terms, we can see
\begin{align*}
    L(X) = \sum_{i = 1}^n \sum_{j = 1}^d (c(X)_{i,j})^2
\end{align*}
Thus we can divide our computation into several steps. To summarize, we first compute the gradients of the pre-defined terms. To be specific, xxx \Yichuan{Chiwun can you fill in our gradient results here?}

Then by decomposing the Hessian into several cases (See Section~\ref{sec:hess_of_loss} for details), we can calculate the final Hessian. \Yichuan{Chiwun can you fill this paragraph? I can improve it based on what you write}

